Graph-Based Fuzz Testing for Deep Learning Inference Engine

With the wide use of Deep Learning (DL) systems, academy and industry begin to pay attention to their quality. Testing is one of the major methods of quality assurance. However, existing testing techniques focus on the quality of DL models but lacks attention to the core underlying inference engines (i.e., frameworks and libraries). Inspired by the success stories of fuzz testing, we design a graph-based fuzz testing method to improve the quality of DL inference engines. This method is naturally followed by the graph structure of DL models. A novel operator-level coverage criterion based on graph theory is introduced and six different mutations are implemented to generate diversified DL models by exploring combinations of model structures, parameters, and data inputs. The Monte Carlo Tree Search (MCTS) is used to drive DL model generation without a training process. The experimental results show that the MCTS outperforms the random method in boosting operator-level coverage and detecting exceptions. Our method has discovered more than 40 different exceptions in three types of undesired behaviors: model conversion failure, inference failure, output comparison failure. The mutation strategies are useful to generate new valid test inputs, by up to 8.2% more operator-level coverage on average and 8.6 more exceptions captured.

==> bug details/MNN x86/mnn_x86_bug_details.tex <==
% 1  DCF-2   已写GH DCF4
% 这个写到支持的数据类型不对

% cast float32 to int8 pymnn没有内部类型支持int8的数据如MNN.Halide_Type_Int8，只有MNN.Halide_Type_Int。而且发现了cast支持uint8 但资料没说支持

% Data Comparison Failure

% read32 fusion_fp16_randomnet_ws_1_431052_0001_test_inputdata_10000_0_fp32.bin
% 2 2 2 2 2 2 2 2
% =============================================================================================
% read_int8 fusion_fp16_randomnet_ws_1_431052_0001_output_cast_outputdata_10000_0_fp32_mnn.bin
% 0 0 1 1 1 1 1 1 
% =============================================================================================
% read_int8 fusion_fp16_randomnet_ws_1_431052_0001_output_cast_outputdata_10000_0_fp32.bin
% 2 2 2 2 2 2 2 2





% 3 dcf  已写 DCF-5

% lrn Data Comparison Failure 

% alpha=1 beta=0.5 bias = 1  depth_raduis=5
% x_data =(np.ones((1,1,1,1))*2).astype(np.float32)
% x_data.tofile(name + "_inputdata_10000_0_fp32.bin")
% out = tf.nn.local_response_normalization(x,name="lrn")
% --------------------------------------------
% Loop     tf_out      mnn_out
% --------------------------------------------
% 1        0.894427        1.712698




% 4  mcf      已写 MCF1

% topkv2  Segmentation fault in TopKV2 conversion
% (gdb) bt
% #0  0x00007f2cc088c6e5 in MNN::TopKV2SizeComputer::onComputeSize(MNN::Op const*, std::vector<MNN::Tensor*, std::allocator<MNN::Tensor*> > const&, std::vector<MNN::Tensor*, std::allocator<MNN::Tensor*> > const&) const () from /usr/local/lib/python2.7/dist-packages/_tools.so
% #1  0x00007f2cc093e84b in MNN::Express::Executor::computeInfo(MNN::Express::Expr*) () from /usr/local/lib/python2.7/dist-packages/_tools.so


% 5  mcf-2 已写  MCF2


% Conversion   aborted.The   deconv   API   of   thepb    model(shown    in    Fig.    8)    is    tf.nn.conv2dtranspose.MNN log: /converter/source/common/writeFb.cpp:108

% mcf-2 pic  resizenearestneighbor+conv2dbackpropinput

% #0  0x00007f9ed925e438 in __GI_raise (sig=sig@entry=6) at ../sysdeps/unix/sysv/linux/raise.c:54
% #1  0x00007f9ed926003a in __GI_abort () at abort.c:89
% #2  0x00007f9ed7d2884d in __gnu_cxx::__verbose_terminate_handler() () from /usr/lib/x86_64-linux-gnu/libstdc++.so.6
% #3  0x00007f9ed7d266b6 in ?? () from /usr/lib/x86_64-linux-gnu/libstdc++.so.6
% #4  0x00007f9ed7d26701 in std::terminate() () from /usr/lib/x86_64-linux-gnu/libstdc++.so.6
% #5  0x00007f9ed7d26919 in __cxa_throw () from /usr/lib/x86_64-linux-gnu/libstdc++.so.6
% #6  0x00007f9e34fdcf9c in writeFb(std::unique_ptr<MNN::NetT, std::default_delete<MNN::NetT> >&, std::string const&, bool, bool) [clone .cold.981] ()
%   from /usr/local/lib/python2.7/dist-packages/_tools.so
% #7  0x00007f9e3500ff59 in PyTool_Converter(_object*, _object*) () at /ruhuan/Projects/AliNNPrivate/pymnn/src/MNNTools.cc:62


% 6  conv2d+deconv   dcf

% Models  Data  Comparison  Failure

% n = 10
% h = 1
% w =3
% c = 3
% x  = tf.placeholder(shape=(n,h,w,c), dtype=tf.float32,name="placeholder_10000")
% x_data = (np.random.rand(n,h,w,c)+1).astype(np.float32)
% x_data.tofile(name + "_inputdata_10000_0_fp32.bin")
% filter_data = np.random.uniform(-1, 1, size=[15,11,3,3]).astype(np.float32) * 0.3  # HWCK
% c = tf.nn.conv2d(x, filter_data,strides=[1,2,1,1],padding='SAME',dilations=[1,1,1,1],name="conv2d")
% filter_data = np.random.uniform(-1, 1, size=[1,3,3,3]).astype(np.float32) * 0.3  # HWCK
% out_2 = tf.nn.conv2d_transpose(c,filter_data, strides=[1,2,2,1],output_shape=[10,2,7,3], padding="VALID",name="deconv")

% the shape of tf output is [10,2,7,3](NHWC), and mnn's is [10,3,1,7] #maybe NCHW and h wrong
% 反卷积valid模式计算时，反卷积出现在网络的中不同的位置，报错现象不一致，
% 但错误原因均为计算outputshape时，c维度计算错误

% 7  IF-1  已写

% a model with 26

% *** Error in `python': free(): invalid next size (fast): 0x0000000001e2cb90 ***
% ======= Backtrace: =========
% /lib/x86_64-linux-gnu/libc.so.6(+0x777f5)[0x7f767300b7f5]
% /lib/x86_64-linux-gnu/libc.so.6(+0x8038a)[0x7f767301438a]
% /lib/x86_64-linux-gnu/libc.so.6(cfree+0x4c)[0x7f767301858c]
% /usr/local/lib/python2.7/dist-packages/_mnncengine.so(_ZN3MNN6TensorD1Ev+0x74)[0x7f7672028654]
% /usr/local/lib/python2.7/dist-packages/_mnncengine.so(+0x4f2a0)[0x7f7671fac2a0]

% #0  0x00007f0c6e11b438 in __GI_raise (sig=sig@entry=6) at ../sysdeps/unix/sysv/linux/raise.c:54
% #1  0x00007f0c6e11d03a in __GI_abort () at abort.c:89
% #2  0x00007f0c6e15d7fa in __libc_message (do_abort=do_abort@entry=2, fmt=fmt@entry=0x7f0c6e276f98 "*** Error in `%s': %s: 0x%s ***\n") at ../sysdeps/posix/libc_fatal.c:175
% #3  0x00007f0c6e16638a in malloc_printerr (ar_ptr=<optimized out>, ptr=<optimized out>, str=0x7f0c6e277010 "free(): invalid next size (fast)", action=3) at malloc.c:5020
% #4  _int_free (av=<optimized out>, p=<optimized out>, have_lock=0) at malloc.c:3874
% #5  0x00007f0c6e16a58c in __GI___libc_free (mem=<optimized out>) at malloc.c:2975
% #6  0x00007f0c6d17a654 in MNN::Tensor::~Tensor() () from /usr/local/lib/python2.7/dist-packages/_mnncengine.so
% #7  0x00007f0c6d0fe2a0 in PyMNNTensor_dealloc (self=0x7f0c6e86ab50) at /ruhuan/Projects/AliNNPrivate/pymnn/src/MNN.cc:1086


% 8 mcf   MCF3
% Models  Conversion  Failure

% *** Error in `/usr/bin/python': free(): invalid pointer: 0x0000000001db1940 ***
% ======= Backtrace: =========
% /lib/x86_64-linux-gnu/libc.so.6(+0x777f5)[0x7f0ed0ec27f5]
% /lib/x86_64-linux-gnu/libc.so.6(+0x8038a)[0x7f0ed0ecb38a]
% /lib/x86_64-linux-gnu/libc.so.6(cfree+0x4c)[0x7f0ed0ecf58c]
% /usr/local/lib/python2.7/dist-packages/_tools.so(_ZNSt15_Sp_counted_ptrIPN3MNN7Express4Expr6InsideELN9__gnu_cxx12_Lock_policyE2EE10_M_disposeEv+0x7e)[0x7                               f0e2cd7cdce]
% /usr/local/lib/python2.7/dist-packages/_tools.so(_ZNSt16_Sp_counted_baseILN9__gnu_cxx12_Lock_policyE2EE10_M_releaseEv+0x47)[0x7f0e2cc46347]
% /usr/local/lib/python2.7/dist-packages/_tools.so(_ZN3MNN7Express4ExprD1Ev+0x25)[0x7f0e2cd7ca95]
% /usr/local/lib/python2.7/dist-packages/_tools.so(_ZNSt15_Sp_counted_ptrIPN3MNN7Express4ExprELN9__gnu_cxx12_Lock_policyE2EE10_M_disposeEv+0x12)[0x7f0e2cd7                               cd32]


% #0  0x00007fd945390438 in __GI_raise (sig=sig@entry=6) at ../sysdeps/unix/sysv/linux/raise.c:54
% #1  0x00007fd94539203a in __GI_abort () at abort.c:89
% #2  0x00007fd9453d27fa in __libc_message (do_abort=do_abort@entry=2, fmt=fmt@entry=0x7fd9454ebf98 "*** Error in `%s': %s: 0x%s ***\n") at ../sysdeps/posix/libc_fatal.c:175
% #3  0x00007fd9453db38a in malloc_printerr (ar_ptr=<optimized out>, ptr=<optimized out>, str=0x7fd9454e8d6f "free(): invalid pointer", action=3) at malloc.c:5020
% #4  _int_free (av=<optimized out>, p=<optimized out>, have_lock=0) at malloc.c:3874
% #5  0x00007fd9453df58c in __GI___libc_free (mem=<optimized out>) at malloc.c:2975
% #6  0x00007fd8a11454a6 in std::string::_Rep::_M_dispose (__a=..., this=<optimized out>) at /opt/rh/devtoolset-8/root/usr/include/c++/8/ext/atomicity.h:82
% #7  std::string::_Rep::_M_dispose (__a=..., this=<optimized out>) at /opt/rh/devtoolset-8/root/usr/include/c++/8/bits/basic_string.h:3250
% #8  std::basic_string<char, std::char_traits<char>, std::allocator<char> >::~basic_string (this=0x12e9320, __in_chrg=<optimized out>)
%     at /opt/rh/devtoolset-8/root/usr/include/c++/8/bits/basic_string.h:3640
% #9  MNN::AttributeT::~AttributeT (this=0x12e9310, __in_chrg=<optimized out>) at /ruhuan/Projects/AliNNPrivate/schema/current/Tensor_generated.h:378
% #10 std::default_delete<MNN::AttributeT>::operator() (this=<optimized out>, __ptr=0x12e9310) at /opt/rh/devtoolset-8/root/usr/include/c++/8/bits/unique_ptr.h:81
% #11 std::default_delete<MNN::AttributeT>::operator() (this=0x12e9648, __ptr=0x12e9310) at /opt/rh/devtoolset-8/root/usr/include/c++/8/bits/unique_ptr.h:75
% #12 std::unique_ptr<MNN::AttributeT, std::default_delete<MNN::AttributeT> >::~unique_ptr (this=0x12e9648, __in_chrg=<optimized out>)
%     at /opt/rh/devtoolset-8/root/usr/include/c++/8/bits/unique_ptr.h:274
% #13 std::_Destroy<std::unique_ptr<MNN::AttributeT, std::default_delete<MNN::AttributeT> > > (__pointer=0x12e9648)
%     at /opt/rh/devtoolset-8/root/usr/include/c++/8/bits/stl_construct.h:98
% #14 std::_Destroy_aux<false>::__destroy<std::unique_ptr<MNN::AttributeT, std::default_delete<MNN::AttributeT> >*> (__last=<optimized out>, __first=0x12e9648)





% 9 % DCF1  gather  已写
% #0  0x00007ff418033438 in __GI_raise (sig=sig@entry=6) at ../sysdeps/unix/sysv/linux/raise.c:54
% #1  0x00007ff41803503a in __GI_abort () at abort.c:89
% #2  0x00007ff4180757fa in __libc_message (do_abort=do_abort@entry=2, fmt=fmt@entry=0x7ff41818ef98 "*** Error in `%s': %s: 0x%s ***\n") at ../sysdeps/posix/libc_fatal.c:175
% #3  0x00007ff41807e38a in malloc_printerr (ar_ptr=<optimized out>, ptr=<optimized out>, str=0x7ff41818f0c8 "double free or corruption (!prev)", action=3) at malloc.c:5020
% #4  _int_free (av=<optimized out>, p=<optimized out>, have_lock=0) at malloc.c:3874
% #5  0x00007ff41808258c in __GI___libc_free (mem=<optimized out>) at malloc.c:2975
% #6  0x00007ff417070098 in MNN::BufferAllocator::Node::~Node() () from /usr/local/lib/python2.7/dist-packages/_mnncengine.so
% #7  0x00007ff4170700c2 in std::_Sp_counted_ptr<MNN::BufferAllocator::Node*, (__gnu_cxx::_Lock_policy)2>::_M_dispose() ()
%   from /usr/local/lib/python2.7/dist-packages/_mnncengine.so
% #8  0x00007ff417070b02 in std::_Rb_tree<unsigned long, std::pair<unsigned long const, std::shared_ptr<MNN::BufferAllocator::Node> >, std::_Select1st<std::pair<unsigned long const, std::shared_ptr<MNN::BufferAllocator::Node> > >, std::less<unsigned long>, std::allocator<std::pair<unsigned long const, std::shared_ptr<MNN::BufferAllocator::Node> > > >::_M_erase(std::_Rb_tree_node<std::pair<unsigned long const, std::shared_ptr<MNN::BufferAllocator::Node> > >*) () from /usr/local/lib/python2.7/dist-packages/_mnncengine.so


% 10
% MCF    MCF4  已写

% Start to Optimize the MNN Net...
% [22:08:40] :20: Inputs: placeholder_10000
% [22:08:40] :37: Outputs: reducesum_outputdata_10400, Type = Reduction

% #0  _int_malloc (av=av@entry=0x7f1376b8ab20 <main_arena>, bytes=bytes@entry=4097) at malloc.c:3619
% #1  0x00007f137684a1d4 in __GI___libc_malloc (bytes=4097) at malloc.c:2920
% #2  0x00000000004a41bf in PyImport_ImportModuleLevel ()
% #3  0x00000000004a5ce4 in ?? ()
% #4  0x00000000004a59e5 in PyObject_CallFunction ()
% #5  0x00000000004a3d27 in PyImport_Import ()
% #6  0x00007f13757dec8e in importName (symbol=0x7f1375a1777f "Tensor", name=0x7f1375a16a3b "MNN") at /ruhuan/Projects/AliNNPrivate/pymnn/src/MNN.cc:50
% #7  0x00007f13757e2912 in PyMNNInterpreter_getSessionOutputAll(PyMNNInterpreter*, _object*) () at /ruhuan/Projects/AliNNPrivate/pymnn/src/MNN.cc:904
% #8  0x00000000004bc9ba in PyEval_EvalFrameEx ()





% 11 cast+slice+reshape  Inference   Failure(IF-2) 这个只能说int32  这个不算问题 slice没说支持，但是支持了，int8是slice不支持的
% ====================================================================================================    Start Reasoning Model.
% The Creator Don't support type [SliceTf], slice
% The Creator Don't support type [SliceTf], slice
% -----------------------------------------------------------------------------------------------------------------------------
% due to the internal logic of MNN, if your MNN model doesn't have input shape, you may ignore this 'Resize error' information:
% ** Resize error for [SliceTf], slice, code=2 **
% it will work after you set the input tensor shape in MNN, and then resize the Session

% 输出的tensor的尺寸为0

% 初步分析可能是cast从float32转成int8时，缩减了分配tensor的内存，
% 导致后续slice错误，如果cast换成int32，则模型正常推理






% 12  dcf  dw
% rn_1_45018_0001
% % output length
% tf:64 bytes  tf shape:(2, 2, 2, 2)
% mnn:32 bytes   output data shape : (8, 1, 1, 1) 

% output_shape = output_tensor[output_name].getShape()
% output_tensor = interpreter.getSessionOutputAll(session)

% n = 2
% h = 2
% w =2
% c =1
% x  = tf.placeholder(shape=(n,h,w,c), dtype=tf.float32,name="placeholder_10000")
% x_data = (np.random.rand(n,h,w,c)+1).astype(np.float32)
% filter = np.random.uniform(-1, 1, size=[1,1,1,2]).astype(np.float32) * 0.8 #hwcn
% padding = 'VALID'
% out = tf.nn.depthwise_conv2d(x,filter,strides = [1,1,1,1],padding = padding,rate = [2,2],name = "depthwise")
% ，（1）由于rate的原因导致，当rate大于1 的时候，filter_n=1 时，计算错误。（2）当filer_n>1 的时候，计算输出维度丢失


% 13 dcf-2   已写

% rsqrt + sigmoid

% rsqrt + sigmoid算子，sigmod算子 tf和mnn中nan处理不一致 tf处理nan为nan mnn处理nan为1 tf处理-inf为0 mnn处理inf为1.64581e-38



14  IF1



15 

==> bug details/TF/tf_bug_details.tex <==
% 1
% When generating a model containing two Concats whose two inputs  come  from  the  same  two  constants,  TensorFlow  will get stuck.
% x_data = (np.ones((n,h,w,c))*2).astype(np.float32)
% x_data.tofile(name + "_input_1.bin")
% y_data = np.random.rand(n,h,w,c).astype(np.float32)
% y=tf.constant(y_data,dtype=tf.float32, shape=(n,h,w,c),name="constant_1")
% m_data = np.random.rand(n,h,w,c).astype(np.float32)
% m=tf.constant(m_data,dtype=tf.float32, shape=(n,h,w,c),name="constant_3")
% c_1= tf.concat([x,y,m], axis=2, name="concat")
% out = tf.concat([c_1,y,m], axis=2, name="concat_1")



% 2
% sqrt+min 
% ***line NO.*****expect******cce*********
% line 0 : 16.0     |  4.0    

% x  = tf.placeholder(shape=(n,h,w,c), dtype=tf.float32,name="input_1")
% x_data = (np.ones((n,h,w,c))*16).astype(np.float32)
% x_data.tofile(name + "_inputdata_10000_0_fp32.bin")
% a = tf.math.sqrt(x,name="sqrt_1")
% res_reducemin_0= tf.reduce_min(a,axis = None,keep_dims = True,name = "redece_0")


% sqrt+min+add(0)
% --------------------------------------------
% Loop 	 Expect_out 	 Real_out
% --------------------------------------------
% 1 	 4.000000 	 4.000000




% 3
% ceil+reducemax
% input [-0.1, 1.6] float32
% % _celi_outputdata_10000_fp32.bin",dtype=np.float32)
% % array([ 1.,  1.,  2.,  1.,  2.,  2.,  2.,  1.,  1.,  1., -0., -0.,  2.,
% %         2.,  2.,  1.,  1.,  2.,  2.,  2.,  1.,  2.,  1., -0.,  1., -0.,
% %         2.,  2.,  1., -0.,  1.,  1.,  1.,  1.,  1.,  1.,  2., -0.,  2.,
% %         2.,  2.,  2.,  1.,  1.,  2.,  1.,  1.,  1.,  1., -0.,  1.,  1.,
% %         1.,  1.,  2.,  1., -0.,  1.,  1.,  1., -0.,  1.,  2.,  1.,  2.,
% %         1.,  2., -0.,  1., -0.,  1.,  1.,  1.,  2.,  2.,  2.,  2.,  1.,

% ceil only  tf=mnn
% reduce max tf = max

% ceil+reducemax output

% >>> np.fromfile("/root/output_reducemax_outputdata_10100_fp32.bin",dtype=np.float32)
% array([1.5992388, 1.5189238, 1.5027162, 1.552708 , 1.5494187, 1.5478246,
%       1.5538496, 1.5889722], dtype=float32)
       
% >>> np.fromfile("/root/output_reducemax_outputdata_10100_fp32_mnn.bin",dtype=np.float32)
% array([2., 2., 2., 2., 2., 2., 2., 2.], dtype=float32)

==> rebuttal.tex <==
We appreciate that the reviewers provide constructive comments. We focus on the major concerns in this letter.
 
** 1. A high-level summary of insights. (Reviewer#1#2) **
Diversified combinations of operators(models) are more capable of triggering DL inference engine issues than individual operators. The issues triggered by a single model are limited. We need to generate a large number of models by combining operators. This paper employs fuzz testing to overcome the challenge of generating models. The detailed high-level summary can be found in Section I. 
 
** 2. The insight behind the operator-level criteria. (Reviewers#1) **
Traditional code coverage criteria are ineffective in DL testing. Recently proposed neuron coverage criteria are still invalid, as DL inference engine testing involves different models. This paper proposes operator-level criteria to capture differences in models combined by operators, which provide feedback to guide the proposed graph-based fuzz testing and generate diversified models. 
 
** 3. The insight behind these found issues. (Reviewer #1#2#3) **
The issues found in this paper indicate that the graph-based fuzz testing for DL inference engine is effective in exposing bugs/crashes. The details of the issues can help developers locate the bugs/crashes by streamlining the model and further improve the quality of inference engines. 
In Fig.8, MCF-2 reveals that the shape of the output tensor calculated by the operator Deconvolution in MNN is wrong.
In Fig.12(b), when given more than 2 inputs, (MS-1(b)) reveals that the operator Concat will lose some of the input data and outputs wrong results.

 
** 4. The generalization of proposed method and threats to validity. (Reviewer #1#3) **
The proposed method is universal and the MNN-based implementation is just one possible application scenario. The method has been used continuously in XXX company(for anonymous reason) for several months, which reduces the internal threats. The external threats to validity are discussed in RQ5. The construct threats to validity are discussed in Section 3.B.
 
** 5. Comparison with the existing fuzz testing. (Reviewer #2) **
Different from existing fuzz testing, our method generates models as the input of the fuzz testing for DL inference engine. Together with the combinations of operators, we design new mutation rules and operator-level criteria to guide fuzz testing. 
 
** 6. Is the MCTS-based approach more effective but not necessarily more efficient? (Reviewer #2#3) **
MCTS search is much effective than random serach. The average unduplicated rate of random search is 11.6\%, which is lower than that of MCTS search(28.3\%). As shown in Table III, our method(Line 2, 3, 4) finds more valid exceptions(Column Exceptions found) during the nightly build in XXX company(for anonymous reason), which is efficient for industry. 
 
** 7. Why did you choose to not have an experiment only with an RN model? (Reviewer #3) **
We do not aim to verify that the RN model is superior to other models. The RN model is only used to generate more diversified models. The experiment shown that the performance of RN is better than that of WS, which will be added in our paper.













We appreciate that the reviewers provide constructive comments. We focus on the major concerns in this letter.
 
**1. A high-level summary of insights. (Reviewer#1#2)**
Diversified combinations of operators(models) are more capable of triggering DL inference engine issues than individual operators. The issues triggered by a single model are limited. We need to generate a large number of models by combining operators. This paper employs fuzz testing to overcome the challenge of generating models. The detailed high-level summary can be found in Section I. 
 
**2. The insight behind the operator-level criteria. (Reviewers#1)**
Traditional code coverage criteria are ineffective in DL testing. Recently proposed neuron coverage criteria are still invalid, as DL inference engine testing involves different models. This paper proposes operator-level criteria to capture differences in models combined by operators, which provide feedback to guide the proposed graph-based fuzz testing and generate diversified models. 
 
**3. The insight behind these found issues. (Reviewer #1#2#3)**
The issues found in this paper indicate that the graph-based fuzz testing for DL inference engine is effective in exposing bugs/crashes. The details of the issues can help developers locate the bugs/crashes by streamlining the model and further improve the quality of inference engines. 
In Fig.8, MCF-2 reveals that the shape of the output tensor calculated by the operator Deconvolution in MNN is wrong.
In Fig.12(b), when given more than 2 inputs, (MS-1(b)) reveals that the operator Concat will lose some of the input data and outputs wrong results.

 
**4. The generalization of proposed method and threats to validity. (Reviewer #1#3)**
The proposed method is universal and the MNN-based implementation is just one possible application scenario. The method has been used continuously in XXX company(for anonymous reason) for several months, which reduces the internal threats. The external threats to validity are discussed in RQ5. The construct threats to validity are discussed in Section 3.B.
 
**5. Comparison with the existing fuzz testing. (Reviewer #2)**
Different from existing fuzz testing, our method generates models as the input of the fuzz testing for DL inference engine. Together with the combinations of operators, we design new mutation rules and operator-level criteria to guide fuzz testing. 
 
**6. Is the MCTS-based approach more effective but not necessarily more efficient? (Reviewer #2#3)**
MCTS search is much effective than random serach. The average unduplicated rate of random search is 11.6\%, which is lower than that of MCTS search(28.3\%). As shown in Table III, our method(Line 2, 3, 4) finds more valid exceptions(Column Exceptions found) during the nightly build in XXX company(for anonymous reason), which is efficient for industry. 
 
**7. Why did you choose to not have an experiment only with an RN model? (Reviewer #3)**
 We do not aim to verify that the RN model is superior to other models. The RN model is only used to generate more diversified models. The experiment shown that the performance of RN is better than that of WS, which will be added in our paper.












1121:

We appreciate that the reviewers provide constructive comments. We focus on the major concerns in this letter.

1. A high-level summary of insights. (Reviewer#1#2) 
1.单个算子/算子组合 触发问题；
2.很难单一网络-大量网络
3.如何生成大量网络？fuzz
Combinations of operators (networks) are more capable of triggering problems than individual operators. The issues triggered by a single network is limited. We need to generate large-scale networks. This paper employs fuzz testing to overcome the challenge of generating networks.


2. The insight behind the operator-level criteria. (Reviewers#1)
不是在单个网络上-新的不可/基于控制的不再有效/需要覆盖到特定的算子组合
传统-基于运行时/本文-基于输入
算子级-可以捕捉到模型的差异/产生多样化的模型
Since the graph-based fuzz testing does not perform on a single network, the criteria that have been proposed in recent years are not suitable. At the same time, the traditional control-based criteria are no longer valid in the input-based fuzz testing. The operator-level criterion can capture the differences in models and lead to the generation of diverse models.

3. The insight behind these found issues. (Reviewer #1#2#3)
问题反映什么问题？单一算子找不到/辅助定位修复/典型问题/精简发现问题的图来定位问题
确定典型问题的分析 2-3个
The details of the issues can be used to locate the cause of the error and help developers improve the operator's quality. We can further localize the problem by streamlining the graph which discovers problem. The issues found in this article are difficult to expose with the single operator. In other words, the graph-based fuzz testing for DL inference engine by combinations of operators is effective.

**补充典型问题**


The shape of the output tensor calculated by the Deconvolution operator in MNN is not the same as that calculated in TensorFlow, which means that the algorithm of the operator implemented by MNN is different from that implemented by TensorFlow(MCF-2).
反卷积算子在MNN中计算的输出张量的大小与在tf中的计算的大小不相同,也就是说MNN实现的该算子的算法与tf实现的有差异。


When the number of inputs is greater than 2, the Concat operator will lose some of the input data and cause the result to be wrong. However, the MNN user guide does not indicate that the Concat operator has the limit on the number of inputs(MS-1(b)).
当输入数大于2时，Concat算子会丢失一些输入的数据，并导致结果错误。但是MNN的用户指导书并未说明Concat算子有输入数的限制。

改了一下 麻烦看看。。。




4. The generalization of proposed method and the threats to validity.(Reviewer #1#3)
框架是统一的，只是基于MNN进行了实现/大规模应用在公司/
The proposed method is universal and the MNN-based implementation is just one possible application scenario. We have already promoted a large-scale application in XXX company(due to Anonymous). 
The internal threat to validity mainly lies in the implementations and our scripts in the study. To reduce this threat, the method has been used continuously in the industry. 
The external threats to validity mainly lie in the used libraries in our study. However, this is a general approach, and it can be used to test other inference engines, which is discussed in RQ5. 
The construct threats to validity mainly lie in measurements in our experiment. The threats from the measurements have been discussed in B of Section 3.


5. Comparison with the existing fuzz testing. (Reviewer #2)
已有的fuzz针对的数据类型与我们不同/
Existing fuzz testing generates different types of data compared with our approach. They generate test data for a specific model, whereas we generate test data in the form of models for inference engines.

6. Is the MCTS-based approach more effective but not necessarily more efficient? (Reviewer #2#3)
从企业的角度来说是可接受的（发现问题+时间接受）。
As shown in Table III, our method(line 2, 3, 4) finds more valid exceptions(Column Exceptions found) in a limited amount of time(Column Duration), which is efficient for the industry.

补充mcts去除重复问题的效果：
The average deduplication rate of random search is 11.6\%, which is lower than the 28\% of MCTS search. The low efficiency of random search is unacceptable.
随机搜索的平均去重的问题发现率为11.6\%，低于MCTS搜索的28\%。随机搜索的低效率是不可接受的。

The total number of issues and the number of deduplicated issues in Table III are reversed. This will be revised in the manuscript.
表3中的问题总数和重复数据删除问题的数目颠倒了。本节将在稿件中进行修改

7. Why did you choose to not have an experiment only with an RN model ?(Reviewer #3)
1.根据结果解释，将来添加结果

1.
The RN model is introduced to show that the richer the graph structures, the richer the models' structures, and to prove the advantages of more models, rather than to verify that the RN model is superior to other models.

补充RN结果：
Based on the configuration parameters in the experiment, when n is 5 and 10, RN is slightly better than WS, and when n is 15, RN and WS are basically the same.

RN mutation：NO     search：MCTS-based   
     OLC            Exceptions found(t/d) Duration(h)
N=5  53.34\%         11.4/78.2               2.6
N=10 58.7\%          15.2/90.8               4.1
N=15 61.4\%          13.5/93                 4.5














======================================================
Threats to validity的补充描述:

The implementation mechanisms of existing DL inference engines are somewhat similar. We used the method in our self-developed DL inference engine testing (Huawei HiAI engine) and found hundreds of issues (e.g. graph optimization errors, operator implementation errors, tiling errors, misuse of instructions). 








=================================================
1119：

Thanks for your careful and valuable comments. We have revised the above-mentioned missing or unclear descriptions in the manuscript.

Reviewer#1:
Q1: Lacking a high-level summary of insights and take away.
A1: Designing an efficient inference engine Fuzzing method is under the great challenges of DL model diversity and a coverage criterion to measure the parts of the inference engine’s logic exercised by a test set.
A novel graph-based fuzz testing method (i.e. model generation, mutations, operator-level coverage criteria) is designed to solve these two challenges.  The method is naturally followed by the graph structure of DL models. 

Q2: Lacking the insight behind the operator-level criteria.
A2: Diversified DL models may trigger errors of different parts of a given DL inference engine. For example, different structures (from graph theory) may trigger data flow processing errors, and different tensor shapes and parameters may trigger operator implementation errors. 
Therefore, the criteria should cover these operator-level test dimensions to guide more effective input DL model generation.

Q3: The insight or clue the reasons behind these found issues.
A3: Those MNN logs (e.g. error codes, stack information), source code, core files, MNN models (e.g. Models  Conversion  Failure), original TensorFlow models, and data of each layer (e.g. Data Comparison Failure) were useful in analyzing reasons. We also generated smaller models to reproduce each issue and verify possible reasons.

Q4: Can the proposed method generalize to other cases? Threats to validity are missing.
A4: Yes. The implementation mechanisms of existing deep learning engines are somewhat similar. We used the method in our self-developed DL inference engine testing and found hundreds of issues (e.g. graph optimization errors, operator implementation errors, tiling errors, misuse of instructions). We will add the discussion in our revised manuscript.


Reviewer#2:
Q1: Presentation issues.
A1: We will correct these issues in our revised manuscript.

Q2: No comparison with the existing fuzz testing.
A2: Existing methods focus on testing specified models, and cannot generate diversified DL models by exploring combinations of model structures, parameters, weights, and inputs.

Q3: The challenges and the RN algorithm are not described properly. 
A3：Please refer to A1 to reviewer#1.  We will correct the issue in our revised manuscript. The example is indeed an actual problem. Please refer to A3 to reviewer#1.

Q4: Lacking the timing results.
A4: The timing results are listed in Table III. Compared with random search, the time spent on MCTS search increased by 44.1\% on average. Mutations and graph models have little effect on overall duration.

Reviewer#3:

Q1: Is the MCTS-based approach more effective but not necessarily more efficient?
A1:  Yes. In extreme cases where only a few test cases are generated, the effect of MCTS search is similar to random search. For example, using a corpus of 100 operators to generate 10 models, and the number of operators included in each model is 5. 
In actual DL learning engine testing, the corpus is usually used to generate hundreds or more models. Therefore, we introduced the MCTS-based search to limit the use of problematic operators to build DL models to reduce repetitive errors and test more deeply.

Q2: Why did you choose to not have an experiment only with an RN model although this would be the most reasonable comparison of the two models?
A2: The RN model is introduced to show that the richer the graph structures, the richer the structures of the models, and to prove the advantages of more models, rather than to prove that the RN model is superior to other models.

Q3: Threats to validity are missing.
A3: Please refer to A4 to reviewer#1.









========================================
1118：

Thanks for your careful and valuable comments. 

Reviewe#1:
Q1: The most important insight drawn.
A1: Designing an efficient inference engine Fuzz testing framework is under the great challenges of DL model diversity and a coverage criterion to measure the parts of a DL inference engine’s logic exercised by a test set and to guide more effective fuzz testing.
A novel graph-based fuzz testing method(i.e. DL model generation, mutations, operator-level coverage criteria ) is designed to generate more diversified DL models effectively.  The method is naturally followed by the graph structure of DL models. 

Q2: The insight behind the operator-level criteria.
A2: Diversified DL models may trigger errors of different structured parts of a given DL inference engine. For example, different structures(from graph theory) may trigger data flow processing errors, and different tensor shapes and parameters may trigger operator implementation errors. 
The input DL models should cover these operator-level test dimensions in the DL inference engine testing. Therefore, the operator-level criteria are defined to guide more effective diversified DL model generation.

Q3: I wonder whether the authors have insight or clue the reasons behind these found issues?
A3: Those MNN logs(e.g. error codes, stack information), source code, core files, MNN models(e.g. Models  Conversion  Failure), original TensorFlow models, and data of each layer(e.g. Data Comparison Failure ) were useful in analyzing reasons.
We also wrote scripts to generate smaller models to reproduce each issue and verify possible reasons.

Q4: Can the proposed method generalize to other cases? Some discussion in Threats to Validity is needed.
A4: Yes. The implementation mechanisms of existing deep learning engines are somewhat similar. We used the method in our self-developed DL inference engine testing and found hundreds of issues(e.g. graph optimization errors, operator implementation errors, tiling errors, misuse of instructions). We will add the discussion in Threats to Validity in our final version.









Reviewe#3:

Q1: Is the MCTS-based approach more effective but not necessarily more efficient?
A1: 
Yes, in extreme cases where only a few test cases are generated, the effect of MCTS search is similar to random search. For example, using a corpus of 100 operators to generate 10 models, and the number of operators included in each model is 5. 
In actual DL learning engine testing, the corpus is usually used to generate thousands of models every day. Therefore, we introduced the MCTS-based search to limit the use of problematic operators to build DL models to reduce repetitive errors and test more deeply.


Q2: Why did you choose to not have an experiment only with an RN model although this would be the most reasonable comparison of the two models?
A2: The RN model is introduced to show that the richer the graph structures, the richer the structures of the models, and to prove the advantages of more models, rather than to prove that the RN model is superior to other models.

Q3: Why did you not discuss threats to validity?
A3: Please refer to A4 to reviewer#1.
